Interaction-via-Actions: Cattle Interaction Detection with Joint Learning of Action-Interaction Latent Space

This paper introduces a method and application for automatically detecting behavioral interactions between grazing cattle from a single image, which is essential for smart livestock management in the cattle industry, such as for detecting estrus. Although interaction detection for humans has been actively studied, a non-trivial challenge lies in cattle interaction detection, specifically the lack of a comprehensive behavioral dataset that includes interactions, as the interactions of grazing cattle are rare events. We, therefore, propose CattleAct, a data-efficient method for interaction detection by decomposing interactions into the combinations of actions by individual cattle. Specifically, we first learn an action latent space from a large-scale cattle action dataset. Then, we embed rare interactions via the fine-tuning of the pre-trained latent space using contrastive learning, thereby constructing a unified latent space of actions and interactions. On top of the proposed method, we develop a practical working system integrating video and GPS inputs. Experiments on a commercial-scale pasture demonstrate the accurate interaction detection achieved by our method compared to the baselines. Our implementation is available at https://github.com/rakawanegan/CattleAct.

==> mlpreamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% mlpreamble.tex
% Matsushita Lab preamble
%
% Created: Aug 6th, 2019
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\RequirePackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} 
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} 
\def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

% Reference commands
\newcommand{\Tref}[1]{Table~\ref{#1}}
\newcommand{\eref}[1]{Eq.~\eqref{#1}}
\newcommand{\Eref}[1]{Equation~\eqref{#1}}
\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\Fref}[1]{Figure~\ref{#1}}
\newcommand{\sref}[1]{Sec.~\ref{#1}}
\newcommand{\Sref}[1]{Section~\ref{#1}}

% Comment commands
\usepackage{xcolor}
\newcounter{todos}
\AtEndDocument{\ifnum\value{todos}>0 \PackageWarning{TODOS}{There are \arabic{todos} todos left in this paper! Fix them before submitting the paper!} \fi}

\newcommand{\naka}[1]{\protect\stepcounter{todos}\textcolor{red}{{[Nakagawa: #1]}}}
\newcommand{\yang}[1]{\protect\stepcounter{todos}\textcolor{teal}{{[Yang: #1]}}}
\newcommand{\fo}[1]{\protect\stepcounter{todos}\textcolor{cyan}{{[FO: #1]}}}
\newcommand{\rs}[1]{\protect\stepcounter{todos}\textcolor{blue}{{[RS: #1]}}}
\newcommand{\todo}[1]{\protect\stepcounter{todos}\textcolor{red}{{[TODO: #1]}}}
\newcommand{\red}[1]{\textcolor{red}{#1}}

% Operators
\newcommand{\argmax}{\mathop{\mathrm{argmax}}\limits}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}\limits}
\newcommand{\rank}[1]{\mathrm{rank}\left(#1\right)}

\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\bignorm}[1]{\bigl\lVert#1\bigr\rVert}
\newcommand{\Bignorm}[1]{\Bigl\lVert#1\Bigr\rVert}
\newcommand{\biggnorm}[1]{\biggl\lVert#1\biggr\rVert}
\newcommand{\Biggnorm}[1]{\Biggl\lVert#1\Biggr\rVert}

% Vector, matrix
\newcommand{\V}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\Vs}[2]{\ensuremath{\mathbf{#1}_\mathrm{#2}}}
\usepackage{bm}
\newcommand{\Vg}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\Vgs}[2]{\ensuremath{\boldsymbol{#1}_\mathrm{#2}}}

%%%%%%%%%%%%%%%%%%%%%%% math variables %%%%%%%%%%%%%%%%%%%%%
\newcommand{\abs}[1]{\lvert#1\rvert}

\newcommand{\diag}{\text{diag}}
\renewcommand{\div}{\text{div$\cdot$}}
% vertical double bars from smallest to largest





